MSRS: Training Multimodal Speech Recognition Models from Scratch with Sparse Mask Optimization

Pre-trained models have been a foundational approach in speech recognition, albeit with associated additional costs. In this study, we propose a regularization technique that facilitates the training of visual and audio-visual speech recognition models (VSR and AVSR) from scratch. This approach, abbreviated as \textbf{MSRS} (Multimodal Speech Recognition from Scratch), introduces a sparse regularization that rapidly learns sparse structures within the dense model at the very beginning of training, which receives healthier gradient flow than the dense equivalent. Once the sparse mask stabilizes, our method allows transitioning to a dense model or keeping a sparse model by updating non-zero values. MSRS achieves competitive results in VSR and AVSR with 21.1% and 0.9% WER on the LRS3 benchmark, while reducing training time by at least 2x. We explore other sparse approaches and show that only MSRS enables training from scratch by implicitly masking the weights affected by vanishing gradients.

==> sections/analysis.tex <==
\subsection{Comparison with other sparse-based training methods}
\label{subsec:ablation}
\input{tables/ablation_pretrainedmodels_small}

We compare various pruning methods for neural networks, focusing on those that achieve the desired sparsity during or at the beginning of training. One such method is Gradual Magnitude Pruning (GMP) \cite{zhu2017prune}, which gradually prunes the smallest magnitude weights during training to reach the target sparsity. Another approach is sparse-to-sparse training, which starts with the target sparsity and uses a prune-and-grow approach to explore the parameter space. Notable methods in this category include SET \cite{mocanu2018scalable}, RigL \cite{evci2020rigging} and CHASE \cite{yin2023dynamic}, which use Erdos-Rényi graphs \cite{mocanu2018scalable} to initialize models at the target sparsity and then prune weights based on magnitude or gradient. Our results show that when a pretrained frontend is given, all sparse strategies function without much degradation, but when the model is randomly initialized, only mask optimization converges. The main difference between mask optimization and other sparse methods is that mask optimization selectively prunes weights that negatively impact the loss, resulting in a narrower model that enables proper gradient flow. In contrast, other sparse methods employ initialization and pruning strategies that are decoupled from the training process. Figure \ref{fig:sparsity_layers} shows the sparsity achieved for each layer using different pruning methods. While Erdos-Rényi initialization primarily targets layers with more weights in the frontend, mask optimization prunes the encoder as well to facilitate gradient flow of deep nets.
\input{figures/sparsity_layers}

\subsection{Impact of pruning speed on training from scratch}
\vspace{-0.1cm}
\label{subsec:lambda}
\input{figures/lambda_analysis}

The success of training speech models from scratch using mask optimization is highly dependent on the hyperparameter $\lambda$. An ablation study has been conducted to investigate the impact of different values of $\lambda$, as shown in Figure \ref{fig:lambda_analysis}. The results indicate that when a good initialization (pretrained frontend) is used, $\lambda$ values within the range of 1e-12 to 1e-7 effectively prune the model to an optimal sparsity of around 40\%. Specifically, larger values of $\lambda$ result in faster pruning but also make recovery more difficult and lead to accuracy drops, while smaller values do not force enough weights to be negative, which will eventually result in a denser model. However, in the context of training from scratch, it is crucial to progressively eliminate weights that hinder the training process by setting to zero those weights that negatively impact the loss until a near-optimal sparsity is attained and a healthier gradient flow is established. Therefore, the target range of $\lambda$ becomes much smaller (1e-10 to 1e-9), with 2e-10 being the best trade-off in our experiments.



==> sections/related_work.tex <==
\section{Related work}
\label{sec:related_work}
\subsection{Network pruning}
Pruning strategies have been extensively studied \cite{hoefler2021sparsity}. Particularly relevant to this work are methods that trim their networks to the desired sparsity either i) during the training process (sparse-during-training), or ii) at the onset of training (sparse-to-sparse). For instance, Zhu et al. \cite{zhu2017prune} introduces  the Gradual Magnitude Pruning (GMP) algorithm that starts from a randomly initialized dense model and gradually prunes the smallest magnitude weights to achieve the target sparsity. Encouragingly, experiments conducted on CNN and sequential LSTM models demonstrate that large-sparse models consistently surpass small-dense models in various tasks with the same memory footprint, while maintaining minimal accuracy loss. Alternatively, sparse-to-sparse methods start with the target sparsity and then use a prune-and-grow approach to dynamically explore the parameter space. Among these, the most notable methods of sparse-to-sparse training are Sparse Evolutionary Training (SET) \cite{mocanu2018scalable} and The Rigged Lottery (RigL) \cite{evci2020rigging}. These models are initialized using Erdos-Rényi (ER) graphs \cite{mocanu2018scalable}, which assign higher sparsities to layers with more parameters and lower sparsities to smaller ones. Subsequently, weights are pruned based on their magnitude and an equal number of parameters are immediately grown, either randomly (in the case of SET) or using the highest gradient magnitude (for RigL). Recently, CHASE \cite{yin2023dynamic} was introduced to execute both unstructured and structured pruning of CNN-based models. For unstructured sparsity, they globally reallocate parameters based on their magnitude and gradient, adhering to a soft memory limit. This approach allows the parameter growth operation to occur prior to the parameter pruning, preventing the removal of important weights. 

\subsection{Supermask and Neural Architecture Search}

On the other hand, some studies discover the existence of Supermasks, masks that can be applied to an untrained, randomly initialized network to produce a model with performance far better than change \cite{ramanujan2020s, zhou2019deconstructing}. 

Similarly, other works \cite{colombo2020disentangling, gao2021adapting, colombo2021differentiable} suggest that instead of pruning based on heuristics (the lowest magnitude weights), subnetworks can be generated by formulating the Neural Architecture Search (NAS) problem as a binary optimization problem. For instance, Gao et al. \cite{gao2021adapting} propose an adapting-by-pruning algorithm exploit the idea that pruning can be formulated as learning how to mask the pre-training model.




==> tables/Architecture_details.tex <==
\begin{table}[tb]
\centering
\label{tab:architecture_details}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{p}} & \multicolumn{4}{c}{\textbf{Encoder}}                                                                                                                                                                                                                                                                                           & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}N layers \\ decoder\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Output \\ MLP\end{tabular}}} \\ \cline{3-6}
                               &                             & \multicolumn{1}{c|}{\textbf{N layers}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Input \\ dimension\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Feed-Forward \\ dimension\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}attention \\ heads\end{tabular}}} &                                                                                       &                                                                                 \\ \midrule
VSR                            & 56 M                        & 12                                     & 256                                                                                      & 2,048                                                                                           & 4                                                                                        & 6                                                                                     & -                                                                               \\
VSR                            & 250 M                       & 12                                     & 768                                                                                      & 3,072                                                                                           & 12                                                                                       & 6                                                                                     & -                                                                               \\
AVSR                           & 268 M                       & 12                                     & 768                                                                                      & 3,072                                                                                           & 12                                                                                       & 6                                                                                     & 768                                                                             \\
AVSR                           & 703 M                       & 20                                     & 1,024                                                                                    & 4,096                                                                                           & 16                                                                                       & 9                                                                                     & 1,024              \\ \bottomrule                                                             
\end{tabular}
}
\end{table}

==> tables/big_setup.tex <==
\begin{table}[hbtp!]

\label{tab:big_setup}
\caption{Sparse BASE-L VSR, ASR and AVSR models evaluated on LRS3. Training data consists of LRS3 or Multiple datasets (LRS3, VoxCeleb2 and AVSpeech). PS: Pruning strategy; MI: Model initialisation.}
\centering
\begin{tabular}{|cccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{PS}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{MI}}} & \multicolumn{2}{c|}{\textbf{LRS3}}                                   & \multicolumn{2}{c|}{\textbf{Multiple}}            \\ \cline{3-6} 
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\textbf{SP}} & \multicolumn{1}{c|}{\textbf{WER}} & \multicolumn{1}{c|}{\textbf{SP}} & \textbf{WER} \\ \hline \hline
\multicolumn{6}{|c|}{\textbf{VSR}}                                                                                                                                                                                \\ \hline
\multicolumn{1}{|c|}{Dense}       & \multicolumn{1}{c|}{Frontend}    & \multicolumn{1}{c|}{0}                & \multicolumn{1}{c|}{36.3}             & \multicolumn{1}{c|}{0}                & 21.1              \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{39.1}             & \multicolumn{1}{c|}{43.8}              & \multicolumn{1}{c|}{39.7}             & 23.2              \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{0}                & \multicolumn{1}{c|}{42.2}              & \multicolumn{1}{c|}{0}                & 21.7              \\ \hline \hline
\multicolumn{6}{|c|}{\textbf{ASR}}                                                                                                                                                                                \\ \hline
\multicolumn{1}{|c|}{Dense}       & \multicolumn{1}{c|}{Frontend}    & \multicolumn{1}{c|}{0}                & \multicolumn{1}{c|}{2.1}               & \multicolumn{1}{c|}{0}                & TO DO             \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{38.2}             & \multicolumn{1}{c|}{2.7}               & \multicolumn{1}{c|}{37.8}             & 1.3               \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{0}                & \multicolumn{1}{c|}{2.3}               & \multicolumn{1}{c|}{0}                & 1.4               \\ \hline \hline
\multicolumn{6}{|c|}{\textbf{AVSR}}                                                                                                                                                                               \\ \hline
\multicolumn{1}{|c|}{Dense}       & \multicolumn{1}{c|}{Frontend}    & \multicolumn{1}{c|}{0}                & \multicolumn{1}{c|}{2.0}               & \multicolumn{1}{c|}{0}                & 1                 \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{39.7}             & \multicolumn{1}{c|}{2.4}               & \multicolumn{1}{c|}{39.7}             & 1.1           \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{0}                & \multicolumn{1}{c|}{2.0}               & \multicolumn{1}{c|}{0}                & 0.9               \\ \hline
\end{tabular}
\end{table}

==> tables/big_setup_all_data.tex <==
\begin{table}[hbtp!]
\label{tab:big_setup_all_data}
\caption{Sparse BASE-L VSR, ASR and AVSR models on LRS3 + VoxCeleb2 + AVSpeech. 
PS: Pruning strategy; MI: Model initialisation.}
\centering
\begin{tabular}{|cccc|}
\hline
\multicolumn{1}{|c|}{\textbf{PS}} & \multicolumn{1}{c|}{\textbf{MI}} & \multicolumn{1}{c|}{\textbf{Sp (\%)}} & \textbf{WER (\%)} \\ \hline
\multicolumn{4}{|c|}{\textbf{VSR}}                                                                                               \\ \hline
\multicolumn{1}{|c|}{Dense}       & \multicolumn{1}{c|}{Frontend}    & \multicolumn{1}{c|}{0}                & 21.1              \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{39.7}             & 23.9              \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{0}                & 21.7              \\ \hline
\multicolumn{4}{|c|}{\textbf{ASR}}                                                                                               \\ \hline
\multicolumn{1}{|c|}{Dense}       & \multicolumn{1}{c|}{Frontend}    & \multicolumn{1}{c|}{0}                & TO DO             \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{37.8}             & 1.3               \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{0}                & 1.4               \\ \hline
\multicolumn{4}{|c|}{\textbf{AVSR}}                                                                                              \\ \hline
\multicolumn{1}{|c|}{Dense}       & \multicolumn{1}{c|}{Frontend}    & \multicolumn{1}{c|}{0}                & 1                 \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{39.7}             & running           \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{0}                & 0.9               \\ \hline
\end{tabular}
\end{table}

==> tables/big_setup_lrs3.tex <==
\begin{table}[hbtp!]
\label{tab:big_setup_lrs3}
\caption{Sparse BASE-L VSR, ASR and AVSR models on LRS3. 
PS: Pruning strategy; MI: Model initialisation.}
\centering
\begin{tabular}{|cccc|}
\hline
\multicolumn{1}{|c|}{\textbf{PS}} & \multicolumn{1}{c|}{\textbf{MI}} & \multicolumn{1}{c|}{\textbf{Sp (\%)}} & \textbf{WER (\%)} \\ \hline \hline
\multicolumn{4}{|c|}{\textbf{VSR}}                                                                                               \\ \hline 
\multicolumn{1}{|c|}{Dense}       & \multicolumn{1}{c|}{Frontend}    & \multicolumn{1}{c|}{0}                & TO DO             \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{39.1}             & 43.8              \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{0}                & 42.2              \\ \hline \hline
\multicolumn{4}{|c|}{\textbf{ASR}}                                                                                               \\ \hline 
\multicolumn{1}{|c|}{Dense}       & \multicolumn{1}{c|}{Frontend}    & \multicolumn{1}{c|}{0}                & 2.1               \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{38.2}             & 2.7               \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{0}                & 2.3               \\ \hline \hline
\multicolumn{4}{|c|}{\textbf{AVSR}}                                                                                              \\ \hline 
\multicolumn{1}{|c|}{Dense}       & \multicolumn{1}{c|}{Frontend}    & \multicolumn{1}{c|}{0}                & 2.0               \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{39.7}             & 2.4               \\ \hline
\multicolumn{1}{|c|}{MaskOpt3}    & \multicolumn{1}{c|}{Random}      & \multicolumn{1}{c|}{0}                & 2.0               \\ \hline
\end{tabular}
\end{table}

